U-Finger: Multi-Scale Dilated Convolutional Network for Fingerprint Image Denoising and Inpainting

This paper studies the challenging problem of fingerprint image denoising and inpainting. To tackle the challenge of suppressing complicated artifacts (blur, brightness, contrast, elastic transformation, occlusion, scratch, resolution, rotation, and so on) while preserving fine textures, we develop a multi-scale convolutional network, termed U- Finger. Based on the domain expertise, we show that the usage of dilated convolutions as well as the removal of padding have important positive impacts on the final restoration performance, in addition to multi-scale cascaded feature modules. Our model achieves the overall ranking of No.2 in the ECCV 2018 Chalearn LAP Inpainting Competition Track 3 (Fingerprint Denoising and Inpainting). Among all participating teams, we obtain the MSE of 0.0231 (rank 2), PSNR 16.9688 dB (rank 2), and SSIM 0.8093 (rank 3) on the hold-out testing set.

==> README <==
            +--------------------------------------------+
            |                FILECONTENTS                |
            |                                            |
            | Improved version of LaTeX2e's filecontents |
            |       and filecontents* environments       |
            |                                            |
            |      By Scott Pakin, scott+fc@pakin.org    |
            +--------------------------------------------+


Description
-----------

LaTeX2e's filecontents and filecontents* environments enable a LaTeX
source file to generate external files as it's run through latex.
However, there are two limitations of these environments: They refuse
to overwrite existing files; and, they can be used only before the
\documentclass declaration.  The filecontents package removes these
limitations, making it possible to overwrite existing files and to use
filecontents/filecontents* anywhere.


Installation
------------

There's nothing special about building filecontents:

    latex filecontents.ins     <== Generate filecontents.sty
    latex filecontents.dtx     <== Produce the documentation (filecontents.dvi)

If you're new to this, see
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=instpackages for more
information on installing packages.


Copyright and license
---------------------

Copyright (C) 2018 Scott Pakin, scott+fc@pakin.org

This package may be distributed and/or modified under the conditions
of the LaTeX Project Public License, either version 1.3c of this
license or (at your option) any later version.  The latest version of
this license is in:

    http://www.latex-project.org/lppl.txt

and version 1.3c or later is part of all distributions of LaTeX
version 2008/05/04 or later.

